Open Challenges and Opportunities in Federated Foundation Models Towards Biomedical Healthcare

This survey explores the transformative impact of foundation models (FMs) in artificial intelligence, focusing on their integration with federated learning (FL) for advancing biomedical research. Foundation models such as ChatGPT, LLaMa, and CLIP, which are trained on vast datasets through methods including unsupervised pretraining, self-supervised learning, instructed fine-tuning, and reinforcement learning from human feedback, represent significant advancements in machine learning. These models, with their ability to generate coherent text and realistic images, are crucial for biomedical applications that require processing diverse data forms such as clinical reports, diagnostic images, and multimodal patient interactions. The incorporation of FL with these sophisticated models presents a promising strategy to harness their analytical power while safeguarding the privacy of sensitive medical data. This approach not only enhances the capabilities of FMs in medical diagnostics and personalized treatment but also addresses critical concerns about data privacy and security in healthcare. This survey reviews the current applications of FMs in federated settings, underscores the challenges, and identifies future research directions including scaling FMs, managing data diversity, and enhancing communication efficiency within FL frameworks. The objective is to encourage further research into the combined potential of FMs and FL, laying the groundwork for groundbreaking healthcare innovations.

==> figures/sys_flfm.tex <==

\begin{figure}[tb]
	\centering
	\begin{subfigure}{0.35\columnwidth}
		\includegraphics[width = 1\columnwidth]{plots/flfm_train.png}
		\caption{FLFM: Training from scratch}
		\label{fig:flfm-train}
	\end{subfigure}
	\begin{subfigure}{0.35\columnwidth}
		\includegraphics[width = 1\columnwidth]{plots/flfm_prompt.png}
		\caption{FLFM: Prompt tuning}
		\label{fig:flfm-prompt}
	\end{subfigure}
	%	\caption{text}
	\caption{Impact of $\rho$ to the proposed BG-Mix and DG-Mix algorithms against the STL-10 and Cifar-100 datasets under the developed G-Mix framework, $\gamma = 0.5$, $|\mathcal{B}|= 512$.}
	\label{fig:sys_flfm}
\end{figure}

==> sections/fm_prompt.tex <==

\section{Prompt Learning}\label{sec:flfm-prompt}
\textcolor{red}{\textbf{Keywords:}} prompt learning, federated learning

Prompt learning is emerging as a pivotal approach in both natural language processing and computer vision fields, enabling models to adapt to new tasks with minimal changes to their architecture or weights. This section explores the integration of prompt learning with federated learning (FL) across different domains, highlighting recent advancements and unique applications.


\paragraph{Prompt Tuning}
Prompt tuning has emerged as a communication-efficient alternative to full model tuning, offering comparable effectiveness \cite{lester2021power}. This approach does not involve sharing the large FM parameters but instead focuses on fine-tuning lightweight, additional tokens—essentially freezing the entire FM's parameters. In federated learning contexts, prompt tuning can leverage the collective knowledge from multiple participants to refine the prompts used in FM training, potentially enhancing FM performance. The method's integration in FL is akin to the adapter approach shown in Figure 5c. Recent research, including studies like FedPrompt \cite{zhao2023fedprompt} and PROMPTFL \cite{guo2023promptfl}, demonstrates the potential of using FL to improve the quality and effectiveness of prompt-based training methods. These studies highlight how FL can enhance prompt tuning without the need to transfer sensitive data or rely on resource-intensive model deployments on user devices. However, they also reveal challenges such as the assumptions of large FMs' availability on user devices, which may not be practical in resource-constrained settings, or potential privacy risks associated with using cloud-based FM APIs. Continuing to explore prompt tuning within FL frameworks could unlock new ways to utilize collective intelligence effectively, thereby optimizing prompts and boosting FM capabilities in various applications.

\paragraph{Other Methods like Model Compression}
Model compression emerges as a crucial strategy to alleviate the significant memory, communication, and computational demands imposed by large foundation models (FMs) \cite{song2023resfed}. By reducing the size of FMs, model compression enables more feasible deployment within federated learning frameworks without markedly diminishing performance. Common compression techniques, such as knowledge distillation \cite{hinton2015distilling}, where a smaller model is trained to mimic the behavior of a larger one, and quantization \cite{yang2019quantization}, which reduces the numerical precision of model parameters to decrease the size and


Furthermore, beyond merely fostering participation, it is crucial to consider how profits and costs associated with deploying FMs via APIs are distributed. Ensuring a fair allocation of rewards and benefits is imperative to maintain trust and promote sustained cooperation among stakeholders. Mechanisms need to be established to define the distribution of profits derived from the use of FMs, guaranteeing a fair share of economic benefits. This equitable distribution is essential not only for fostering a sense of fairness but also for encouraging continued participation and investment in the FL ecosystem for FMs.ss

\subsection{FL on Large Language Models}
\textcolor{red}{\textbf{Keywords:}} GPT-fl

The integration of federated learning with large language models through prompt learning offers new methodologies for enhancing model adaptability without compromising user privacy. One notable implementation in this domain is \textit{GPT-fl} by Zhang et al., which utilizes prompt learning techniques within a federated framework to allow language models to efficiently learn from decentralized datasets \cite{zhang2023gpt}. This approach not only maintains the privacy of the data but also leverages the inherent flexibility of prompt-based methods to improve model performance across a variety of linguistic tasks.

\subsection{FL on Vision Language Models}
\textcolor{red}{\textbf{Keywords:}} vision language model, prompt learning

In the context of vision language models, federated learning combined with prompt learning techniques is gaining traction as a method for training models on distributed visual and textual data. Innovations such as \textit{PromptFL} by Guo et al. \cite{guo2023promptfl} and a contrastive learning approach for federated learning from pre-trained models \cite{tan2022federated} are leading the way in this field. These methods enable models to handle complex multimodal tasks by learning efficient representations and alignments between text and image data in a privacy-preserving manner.

Further developments include \textit{FedPrompt}, \textit{FedTPG}, and \textit{pFedPrompt}, which are various approaches exploring how to optimize prompt-based training strategies within federated settings. These techniques demonstrate the potential to enhance the usability and efficiency of vision language models under the constraints of federated learning.

This section underscores the crucial role of prompt learning in expanding the capabilities of both language and vision models trained in federated environments. By facilitating efficient task adaptation and maintaining data privacy, prompt learning represents a significant step forward in the development of AI systems that can operate across diverse and distributed data landscapes.

